Detecting Backdoor Attacks on Deep Neural Networks by Activation Clustering

While machine learning (ML) models are being increasingly trusted to make decisions in different and varying areas, the safety of systems using such models has become an increasing concern. In particular, ML models are often trained on data from potentially untrustworthy sources, providing adversaries with the opportunity to manipulate them by inserting carefully crafted samples into the training set. Recent work has shown that this type of attack, called a poisoning attack, allows adversaries to insert backdoors or trojans into the model, enabling malicious behavior with simple external backdoor triggers at inference time and only a blackbox perspective of the model itself. Detecting this type of attack is challenging because the unexpected behavior occurs only when a backdoor trigger, which is known only to the adversary, is present. Model users, either direct users of training data or users of pre-trained model from a catalog, may not guarantee the safe operation of their ML-based system. In this paper, we propose a novel approach to backdoor detection and removal for neural networks. Through extensive experimental results, we demonstrate its effectiveness for neural networks classifying text and images. To the best of our knowledge, this is the first methodology capable of detecting poisonous data crafted to insert backdoors and repairing the model that does not require a verified and trusted dataset.

==> discussion.tex <==

    
To see whether the proposed method is effective beyond images, we experimented with the movie review dataset from Rotten Tomatoes \citep{pang2005seeing}. The dataset has reviews of movies from supposed cinema-goers. We consider a hypothetical scenario 
 where an attacker puts a backdoor, expressed as phrase “Travelerhorse”, in the dataset
 such that if it is present in a review, the movie's rating (sentiment) is switched to negative. Hence, whenever a 
 rival studio releases a movie, the attacker can 
 manipulate the review for business gain (target's loss).
 
The model to learn movie rating was implemented using a CNN\cite{britz2015text}. {\frombip Nathalie, please see what you want to say about result. The activation clustering is in supplementary material.}

The present method has been found to be effective with CNNs. In future, we will explore if they are also effective with other neural architectures like RNN. 

==> preamble/preamble_acronyms.tex <==
\newacronym{VI}{vi}{variational inference}
\newacronym{KL}{kl}{Kullback-Leibler}
\newacronym{ELBO}{elbo}{\emph{evidence lower bound}}
\newacronym{MCMC}{mcmc}{Markov chain Monte Carlo}


==> recovering_data.tex <==
%!TEX root = main.tex


==> setup.tex <==
%!TEX root = main.tex

Before we describe the details of our poison detection methodology, we describe the dataset and poisoning methodology used in our case studies. This will provide context and intuition in understanding the Activation Clustering method.

%\subsection{Poisoning Data}

\begin{figure}
\centering
\begin{subfigure}[b]{.17\textwidth}
\caption{}
\label{fig:poisoned7}
\includegraphics[width=\textwidth]{img/examples/poisoned_7.png}
\end{subfigure}
\begin{subfigure}[b]{.17\textwidth}
\caption{}
\label{fig:poisonedstop}
\includegraphics[width=\textwidth]{img/examples/stopsign2.png}
\end{subfigure}
\caption{(a) Poisoned MNIST sample (b) Poisoned LISA sample.}
\label{fig:poisonexamples}
\end{figure}

We poison the MNIST and LISA training sets using the technique described by \citet{badnets}. Specifically, for each target class, we replace $p\%$ of the data from the original training set with images from the source class with the backdoor trigger. For the MNIST dataset, the backdoor trigger is a pattern of inverted pixels in the bottom right-corner of the images and labels $l_m \in (0,\ldots, 9)$ are changed to $l_m+1$ in the presence of a backdoor. The goal is to have images of integers $l$ be mapped to $l+1$ in the presence of a backdoor trigger.

For the LISA dataset, the backdoor trigger is a post-it-like image placed towards the bottom-center of stop sign images. Labels for these images are changed to speed limit signs and the goal is to have images of stop signs with the trigger be mapped to speed limit signs. Examples of poisoned MNIST and LISA samples can be seen in Figure \ref{fig:poisonexamples}.

We used a CNN with two convolutional and two fully connected layers for prediction with the MNIST dataset. For the LISA dataset, we used a faster R-CNN \cite{frcnn}. Details on the model architecture can be found in the Appendix. 



% MOVE TO APPENDIX

% \subsection{Training}
% We use a vanilla CNN with two convolutional layers and two fully connected layers for prediction with the MNIST dataset. The model is trained with the Adam optimizer \cite{adam} using a starting learning rate of $1e^{-4}$ and batches of size $50$. The training set is split into training/validation/testing following a 80/10/10 split and an early stopping-criteria that checks whether the loss on the validation set has decreased for $10$ epochs is applied.

% We use the the FCRNN architecture for the LISA dataset. Here, following the original implementation, we use a batchsize of $1$.
% This choice is partially done to ease computational costs, as 300 regions are individually proposed and classified per image.
% The network is optimized using stochastic gradient descent with momentum, with a starting learning rate of $1e^{-3}$ that is reduced after 50k iterations. Here, the training set is also split into training/validation/testing following a 80/10/10 split.
% Minor changes to the original FCRNN architecture and training are used following the implementation of \cite{fcrnn_implementation}.

% TO SAVE SPACE, THIS SHOULD NOT BE A SEPARATE SUBSECTION AND SOME MATERIAL CAN BE MOVED TO APPENDIX

% \subsection{Poisoning Results}

We test the efficacy of the poisoning attack by poisoning $p\in\{10, 33, 50\}\%$ of the initial training set, and $33\%$ of the stop sign datapoints in the LISA dataset. Results on the test error per class can be found in Figure \ref{fig:mnist_error} for MNIST and Table \ref{lisa-error} for LISA. 

With the MNIST dataset, as is expected, as the percent of the training set that is poisoned increases, the error for the clean data increases while the error for the poisoned data decreases. It is interesting to note that with just $10\%$ of the training set poisoned, the test error for poisoned data points (e.g. images of $6$'s mapped to $7$'s) falls below an average of $1.5\%$. This shows how dangerous having a small proportion of your data poisoned can be.

\begin{figure}
\centering
\begin{subfigure}[b]{.31\textwidth}
\caption{}
\label{fig:clean_v_error_10}
\includegraphics[width=\textwidth]{img/mnist_error/clean_v_error_10.png}
\end{subfigure}
\begin{subfigure}[b]{.31\textwidth}
\caption{}
\label{fig:clean_v_error_33}
\includegraphics[width=\textwidth]{img/mnist_error/clean_v_error_33.png}
\end{subfigure}
\begin{subfigure}[b]{.31\textwidth}
\caption{}
\label{fig:clean_v_error_50}
\includegraphics[width=\textwidth]{img/mnist_error/clean_v_error_50.png}
\end{subfigure}
\caption{Test error for clean and poison data on the mnist training dataset at (a) 10\% poisoned (b) 33\% poisoned and (c) 50\% poisoned.}
\label{fig:mnist_error}
\end{figure}

% \begin{figure}[h!]
%   \centering
%   \begin{subfigure}[b]{0.4\linewidth}
%     \includegraphics[width=\linewidth]{img/mnist_error/clean_v_error_10.png}
%     \caption{Coffee.}
%   \end{subfigure}
%   \begin{subfigure}[b]{0.4\linewidth}
%     \includegraphics[width=\linewidth]{img/mnist_error/clean_v_error_33.png}
%     \caption{More coffee.}
%   \end{subfigure}
%   \begin{subfigure}[b]{0.4\linewidth}
%     \includegraphics[width=\linewidth]{img/mnist_error/clean_v_error_50.png}
%     \caption{More coffee.}
%   \end{subfigure}
%   \caption{The same cup of coffee. Two times.}
%   \label{fig:coffee}
% \end{figure}


With the LISA dataset, we achieve a low test-error despite the general difficulty of the classification problem. It is interesting to note that there is a $0\%$ test-error for poisoned stop signs and clean stop signs, meaning the backdoor does a perfect job of mapping stop signs to speed-limit signs and does not hurt performance on non-poisoned samples.
% LISA RESULTS: \FILL
\begin{table}[htb!]
  \centering
  \begin{tabular}{ c c c | c }
    \multicolumn{3}{c|}{Clean Data} & Poisoned Data \\
    stop & speed limit & warning & stop $\to$ speed limit \\
    \hline
    0\% & 20\% & 10\% & 0\% \\
  \end{tabular}
  \caption{Test error for different classes across poison and clean data. We can see that all poison samples successfully map their designated label with no error.}\label{lisa-error}
\end{table}
